Next-to-leading order scalar contributions to $\mu\rightarrow e$ conversion

Within a class of models in which lepton flavor violation is induced dominantly by scalar particle exchanges, we estimate the $\mu \to e$ conversion rate in several nuclei. We include next-to-leading order (NLO) terms in the one- and two-nucleon interactions in chiral effective theory, rectifying some incorrect results in the previous literature. We provide an uncertainty budget for the conversion rates and we find that NLO contributions affect the amplitudes at the level of $10\%$, which could be larger than the uncertainty on the leading order couplings, dominated by the strange and non-strange nucleon sigma terms. We study the implications of our results for testing Higgs-mediated CLFV in the future by combining results from various experimental searches, such as $\mu \to e$ conversion in multiple target nuclei and $\mu \to e \gamma$.

==> bib.tex <==
%Reference
\begin{thebibliography}{99}
%
%------------------------------------- Introduction ---------------------------------------
%\cite{MEG:2016leq}
\bibitem{MEG:2016leq}
A.~M.~Baldini \textit{et al.} [MEG],
%``Search for the lepton flavour violating decay $\mu ^+ \rightarrow \mathrm {e}^+ \gamma $ with the full dataset of the MEG experiment,''
Eur. Phys. J. C \textbf{76}, no.8, 434 (2016)
%doi:10.1140/epjc/s10052-016-4271-x
%[arXiv:1605.05081 [hep-ex]].
%701 citations counted in INSPIRE as of 20 Nov 2021

%\cite{SINDRUMII:2006dvw}
\bibitem{SINDRUMII:2006dvw}
W.~H.~Bertl \textit{et al.} [SINDRUM II],
%``A Search for muon to electron conversion in muonic gold,''
Eur. Phys. J. C \textbf{47}, 337-346 (2006)
%doi:10.1140/epjc/s2006-02582-x
%603 citations counted in INSPIRE as of 20 Nov 2021

%\cite{MEGII:2018kmf}
\bibitem{MEGII:2018kmf}
A.~M.~Baldini \textit{et al.} [MEG II],
%``The design of the MEG II experiment,''
Eur. Phys. J. C \textbf{78}, no.5, 380 (2018)
%doi:10.1140/epjc/s10052-018-5845-6
%[arXiv:1801.04688 [physics.ins-det]].
%174 citations counted in INSPIRE as of 20 Nov 2021

%\cite{MEGII:2021fah}
\bibitem{MEGII:2021fah}
A.~M.~Baldini \textit{et al.} [MEG II],
%``The Search for \ensuremath{\mu}+ \textrightarrow{} e+\ensuremath{\gamma} with 10\textendash{}14 Sensitivity: The Upgrade of the MEG Experiment,''
Symmetry \textbf{13}, no.9, 1591 (2021)
%doi:10.3390/sym13091591
%[arXiv:2107.10767 [hep-ex]].
%3 citations counted in INSPIRE as of 20 Nov 2021

%\cite{Diociaiuti:2020yvo}
\bibitem{Diociaiuti:2020yvo}
E.~Diociaiuti,
%``$\mu \rightarrow e$ conversion and the Mu2e experiment at Fermilab,''
PoS \textbf{EPS-HEP2019}, 232 (2020)
%doi:10.22323/1.364.0232
%1 citations counted in INSPIRE as of 20 Nov 2021

%\cite{Moritsu:2021fns}
\bibitem{Moritsu:2021fns}
M.~Moritsu [COMET],
%``The COMET Experiment: Search for Muon-to-Electron Conversion,''
JPS Conf. Proc. \textbf{33}, 011111 (2021)
%doi:10.7566/JPSCP.33.011111
%2 citations counted in INSPIRE as of 20 Nov 2021


%------------------------------------- Lagrangian ---------------------------------------

%\cite{Weinberg:1979sa}
\bibitem{Weinberg:1979sa}
S.~Weinberg,
%``Baryon and Lepton Nonconserving Processes,''
Phys. Rev. Lett. \textbf{43}, 1566-1570 (1979)
doi:10.1103/PhysRevLett.43.1566
%1955 citations counted in INSPIRE as of 23 Oct 2021

%\cite{Wilczek:1979hc}
\bibitem{Wilczek:1979hc}
F.~Wilczek and A.~Zee,
%``Operator Analysis of Nucleon Decay,''
Phys. Rev. Lett. \textbf{43}, 1571-1573 (1979)
doi:10.1103/PhysRevLett.43.1571
%562 citations counted in INSPIRE as of 23 Oct 2021

%\cite{Buchmuller:1985jz}
\bibitem{Buchmuller:1985jz}
W.~Buchmuller and D.~Wyler,
%``Effective Lagrangian Analysis of New Interactions and Flavor Conservation,''
Nucl. Phys. B \textbf{268}, 621-653 (1986)
doi:10.1016/0550-3213(86)90262-2
%1942 citations counted in INSPIRE as of 23 Oct 2021



%\cite{Grzadkowski:2010es}
\bibitem{Grzadkowski:2010es}
B.~Grzadkowski, M.~Iskrzynski, M.~Misiak and J.~Rosiek,
%``Dimension-Six Terms in the Standard Model Lagrangian,''
JHEP \textbf{10}, 085 (2010)
doi:10.1007/JHEP10(2010)085
[arXiv:1008.4884 [hep-ph]].
%1474 citations counted in INSPIRE as of 23 Oct 2021


%\cite{Kitano:2002mt}
\bibitem{Kitano:2002mt}
R.~Kitano, M.~Koike and Y.~Okada,
%``Detailed calculation of lepton flavor violating muon electron conversion rate for various nuclei,''
Phys. Rev. D \textbf{66}, 096002 (2002)
%doi:10.1103/PhysRevD.76.059902
%[arXiv:hep-ph/0203110 [hep-ph]].
%281 citations counted in INSPIRE as of 19 Apr 2020

%\cite{Cirigliano:2009bz}
\bibitem{Cirigliano:2009bz}
V.~Cirigliano, R.~Kitano, Y.~Okada and P.~Tuzon,
%``On the model discriminating power of mu ---> e conversion in nuclei,''
Phys. Rev. D \textbf{80}, 013002 (2009)
%doi:10.1103/PhysRevD.80.013002
%[arXiv:0904.0957 [hep-ph]].
%95 citations counted in INSPIRE as of 19 Apr 2020


%\cite{Shifman:1978zn}
\bibitem{Shifman:1978zn}
M.~A.~Shifman, A.~I.~Vainshtein and V.~I.~Zakharov,
%``Remarks on Higgs Boson Interactions with Nucleons,''
Phys. Lett. B \textbf{78}, 443-446 (1978)
doi:10.1016/0370-2693(78)90481-1
%585 citations counted in INSPIRE as of 21 Oct 2021




%\cite{Cirigliano:2012pq}
\bibitem{Cirigliano:2012pq}
V.~Cirigliano, M.~L.~Graesser and G.~Ovanesyan,
%``WIMP-nucleus scattering in chiral effective theory,''
JHEP \textbf{10}, 025 (2012)
doi:10.1007/JHEP10(2012)025
[arXiv:1205.2695 [hep-ph]].
%101 citations counted in INSPIRE as of 21 Oct 2021

%\cite{Crivellin:2013ipa}
\bibitem{Crivellin:2013ipa}
A.~Crivellin, M.~Hoferichter and M.~Procura,
%``Accurate evaluation of hadronic uncertainties in spin-independent WIMP-nucleon scattering: Disentangling two- and three-flavor effects,''
Phys. Rev. D \textbf{89}, 054021 (2014)
doi:10.1103/PhysRevD.89.054021
[arXiv:1312.4951 [hep-ph]].
%146 citations counted in INSPIRE as of 21 Oct 2021

%\cite{Crivellin:2014cta}
\bibitem{Crivellin:2014cta}
A.~Crivellin, M.~Hoferichter and M.~Procura,
%``Improved predictions for $\mu\to e$ conversion in nuclei and Higgs-induced lepton flavor violation,''
Phys. Rev. D \textbf{89}, 093024 (2014)
doi:10.1103/PhysRevD.89.093024
[arXiv:1404.7134 [hep-ph]].
%62 citations counted in INSPIRE as of 21 Oct 2021


%\cite{Korber:2017ery}
\bibitem{Korber:2017ery}
C.~K\"orber, A.~Nogga and J.~de Vries,
%``First-principle calculations of Dark Matter scattering off light nuclei,''
Phys. Rev. C \textbf{96}, no.3, 035805 (2017)
doi:10.1103/PhysRevC.96.035805
[arXiv:1704.01150 [hep-ph]].
%43 citations counted in INSPIRE as of 21 Oct 2021


%\cite{Bartolotta:2017mff}
\bibitem{Bartolotta:2017mff}
A.~Bartolotta and M.~J.~Ramsey-Musolf,
%``Coherent $\mu-e$ conversion at next-to-leading order,''
Phys. Rev. C \textbf{98}, no.1, 015208 (2018)
%doi:10.1103/PhysRevC.98.015208
%[arXiv:1710.02129 [hep-ph]].
%6 citations counted in INSPIRE as of 19 Apr 2020




%\cite{Hoferichter:2015dsa}
\bibitem{Hoferichter:2015dsa}
M.~Hoferichter, J.~Ruiz de Elvira, B.~Kubis and U.~G.~Mei\ss{}ner,
%``High-Precision Determination of the Pion-Nucleon \ensuremath{\sigma} Term from Roy-Steiner Equations,''
Phys. Rev. Lett. \textbf{115}, 092301 (2015)
doi:10.1103/PhysRevLett.115.092301
[arXiv:1506.04142 [hep-ph]].
%199 citations counted in INSPIRE as of 23 Oct 2021

%\cite{Brantley:2016our}
\bibitem{Brantley:2016our}
D.~A.~Brantley, B.~Joo, E.~V.~Mastropas, E.~Mereghetti, H.~Monge-Camacho, B.~C.~Tiburzi and A.~Walker-Loud,
%``Strong isospin violation and chiral logarithms in the baryon spectrum,''
[arXiv:1612.07733 [hep-lat]].
%27 citations counted in INSPIRE as of 23 Oct 2021


%\cite{Borsanyi:2014jba}
\bibitem{Borsanyi:2014jba}
S.~Borsanyi, S.~Durr, Z.~Fodor, C.~Hoelbling, S.~D.~Katz, S.~Krieg, L.~Lellouch, T.~Lippert, A.~Portelli and K.~K.~Szabo, \textit{et al.}
%``Ab initio calculation of the neutron-proton mass difference,''
Science \textbf{347}, 1452-1455 (2015)
doi:10.1126/science.1257050
[arXiv:1406.4088 [hep-lat]].
%309 citations counted in INSPIRE as of 23 Oct 2021

%\cite{Bernard:1992qa}
\bibitem{Bernard:1992qa}
V.~Bernard, N.~Kaiser, J.~Kambor and U.~G.~Meissner,
%``Chiral structure of the nucleon,''
Nucl. Phys. B \textbf{388}, 315-345 (1992)
doi:10.1016/0550-3213(92)90615-I
%538 citations counted in INSPIRE as of 23 Oct 2021

%\cite{Hoferichter:2012wf}
\bibitem{Hoferichter:2012wf}
M.~Hoferichter, C.~Ditsche, B.~Kubis and U.~G.~Meissner,
%``Dispersive analysis of the scalar form factor of the nucleon,''
JHEP \textbf{06}, 063 (2012)
doi:10.1007/JHEP06(2012)063
[arXiv:1204.6251 [hep-ph]].
%99 citations counted in INSPIRE as of 23 Oct 2021



%\cite{FlavourLatticeAveragingGroup:2019iem}
\bibitem{FlavourLatticeAveragingGroup:2019iem}
S.~Aoki \textit{et al.} [Flavour Lattice Averaging Group],
%``FLAG Review 2019: Flavour Lattice Averaging Group (FLAG),''
Eur. Phys. J. C \textbf{80}, no.2, 113 (2020)
doi:10.1140/epjc/s10052-019-7354-7
[arXiv:1902.08191 [hep-lat]].
%554 citations counted in INSPIRE as of 23 Oct 2021





%------------------------------------- Transition rate ---------------------------------------
\bibitem{Rose1961}
M. E. Rose. Relativistic Electron Theory. John Wiley $\&$ Sons, Inc., New York and London, 1961.

\bibitem{Strange1998}
P. Strange. Relativistic Quantum Mechanics. Cambridge University Press, 1998.

%\cite{Silbar:2010wx}
\bibitem{Silbar:2010wx}
R.~R.~Silbar and T.~Goldman,
%``Solving the radial Dirac equations: A Numerical odyssey,''
Eur. J. Phys. \textbf{32}, 217-233 (2011)
%doi:10.1088/0143-0807/32/1/021
%[arXiv:1001.2514 [physics.comp-ph]].
%8 citations counted in INSPIRE as of 23 Apr 2020

\bibitem{Garcia-Recio1992}
C. Garcia-Recio, J. Nieves, and E. Oset, Nucl. Phys. A 547, 473 (1992).

\bibitem{Vries1987}
H. De Vries, C. De Jager, and C. De Vries, At. Data Nucl. Data Tables 36, 495 (1987).

%------------------------------------- Results ---------------------------------------

%\cite{Harnik:2012pb}
\bibitem{Harnik:2012pb}
R.~Harnik, J.~Kopp and J.~Zupan,
%``Flavor Violating Higgs Decays,''
JHEP \textbf{03} (2013), 026
%doi:10.1007/JHEP03(2013)026
%[arXiv:1209.1397 [hep-ph]].
%319 citations counted in INSPIRE as of 17 Aug 2021

\bibitem{ICHEPMu2E}
M.~ Yucel, ``Muon to electron conversion search in the presence of Al nuclei at the Fermilab Mu2e experiment: Motivation, Design and Progress'', ICHEP 2020 July 28 -- August 6.

\bibitem{ICHEPCOMET}
H.~Nishiguchi, ``The COMET experiment: A search for muon-to-electron conversion at J-PARC'', ICHEP 2020, July 28 -- August 6.

%----------------------------GXFP1 Shell Model Interaction     -----------------------------

%\cite{GXPF1}
\bibitem{GXPF1} M. Honma, T. Otsuka, B. A. Brown, and T. Mizusaki, Phys. Rev. C {\bf 65} (2004) 061301 and
Phys. Rev. C {\bf 69} (2005) 034335.

%----------------------------USDB Shell Model Interaction     -----------------------------

%\cite{USDB}
\bibitem{USDB} B. A. Brown and W. A. Richter, Phys. Rev. C {\bf 74} (2006) 034315.

%----------------------------anapole moment                  -----------------------------

%\cite{anapole}
\bibitem{anapole} Haxton, W. C., Liu, C.-P., and Ramsey-Musolf, M. J., Phys. Rev. C, {\bf 65} (2002) 045502.

%----------------------------bigstick code           -----------------------------

%\cite{bigstick1}
\bibitem{bigstick1} C. W. Johnson, W. E. Ormand, and P. G. Krastev, Comp. Phys. Comm. {\bf 184}, 2671 (2013).

%\cite{bigstick2}
\bibitem{bigstick2} C. W. Johnson, W. E. Ormand, K. S. McElvain, and H. Shan, arXiv:1801.08432.


%----------------------------    correlation function     -----------------------------

%\cite{miller}
\bibitem{miller} Gerald A. Miller and James E. Spencer, Annals of Physics, 100(1):562-606 (1976).

%----------------------------fermi momentum     -----------------------------

%\cite{moniz}
\bibitem{moniz} Moniz, E. J. and Sick, I. and Whitney, R. R. and Ficenec, J. R. and Kephart, R. D. and Trower, W. P., Phys. Rev. Lett. {\bf 26}, 445 (1971).

%----------------------------0vbb operator---------------------------
%\cite{prezeau}
\bibitem{prezeau} Prézeau, G., Ramsey-Musolf, M., and Vogel, P., Phys. Rev. D, {\bf 68}, 034016 (2003).

%----------------------------nucleon sigma lattice--------------------
%\cite{gupta}
\bibitem{gupta} Gupta, R., Park, S., Hoferichter, M., Mereghetti, E., Yoon, B., and Bhattacharya, T., arXiv:2105.12095.

\end{thebibliography}
